Closed-form mathematical expressions for the exponentiated Cauchy-Rayleigh distribution

The Cauchy-Rayleigh (CR) distribution has been successfully used to describe asymmetric and heavy-tail events from radar imagery. Employing such model to describe lifetime data may then seem attractive, but some drawbacks arise: its probability density function does not cover non-modal behavior as well as the CR hazard rate function (hrf) assumes only one form. To outperform this difficulty, we introduce an extended CR model, called exponentiated Cauchy-Rayleigh (ECR) distribution. This model has two parameters and hrf with decreasing, decreasing-increasing-decreasing and upside-down bathtub forms. In this paper, several closed-form mathematical expressions for the ECR model are proposed: median, mode, probability weighted, log-, incomplete and order statistic moments and Fisher information matrix. We propose three estimation procedures for the ECR parameters: maximum likelihood (ML), bias corrected ML and percentile-based methods. A simulation study is done to assess the performance of estimators. An application to survival time of heart problem patients illustrates the usefulness of the ECR model. Results point out that the ECR distribution may outperform classical lifetime models, such as the gamma, Birnbaun-Saunders, Weibull and log-normal laws, before heavy-tail data.

==> glossaries-entries.tex <==
\newentry{cfS}{
  name=\ensuremath{\sym{cfS}_X(t)=\sym{E}(\e^{itX})},
  description={\Al{cf} of a \al{rv} $X$},
  text={characteristic function},
  category=symbol,
  type=symbols,
  sort={cf},
  symbol=\ensuremath{\varphi}
}
\newentry{pdfS}{
  name=\ensuremath{\sym{pdfS}_X(x)=\displaystyle\frac{\mathrm{d}}{\mathrm{d}x}\sym{cdfS}_X(x)},
  description={\Al{pdf} of a continuous \al{rv} $ X $},
  text={probability density function},
  category=symbols,
  type=symbols,
  sort={pdf1},
  symbol=\ensuremath{f}
}
\newentry{bpdfS}{
  name=\ensuremath{\sym{bpdfS}_X(x)=\sym{pdfS}_X(x)},
  description={Baseline \al{pdf} of a continuous \al{rv} $ X $},
  text={baseline probability density function},
  category=symbol,
  type=symbols,
  sort={pdf2},
  symbol=\ensuremath{g}
}
\newentry{cdfS}{
  name=\ensuremath{\sym{cdfS}_X(x)=\sym{Pr}(X\le x)},
  description={\Al{cdf} of a \al{rv} $ X $},
  text={cumulative distribution function},
  category=symbol,
  type=symbols,
  sort={cdf1},
  symbol=\ensuremath{F}
}
\newentry{bcdfS}{
  name=\ensuremath{\sym{bcdfS}_X(x)=\sym{cdfS}_X(x)},
  description={Baseline \al{cdf} of a \al{rv} $ X $},
  text={baseline cumulative distribution function},
  category=symbol,
  type=symbols,
  sort={cdf2},
  symbol=\ensuremath{G}
}
\newentry{qfS}{
  name=\ensuremath{\sym{qfS}_X(p)=\inf\{x\in\sym{Re};p\le\sym{cdfS}_X(x)\}},
  description={\Al{qf} of a \al{rv} $X$.},
  text={quantile function}
  category=symbol,
  type=symbols,
  sort={qf},
  symbol=\ensuremath{Q}
}
\newentry{rhrfS}{
  name=\ensuremath{\sym{rhrfS}_X(t)=\dfrac{\sym{pdfS}_X(x)}{\sym{cdfS}_X(x)}},
  description={\Al{rhrf} of a \al{rv} $ X $.},
  text={reverse hazard rate function},
  category=symbols,
  type=symbols,
  sort={hrf2},
  symbol=\ensuremath{r}
}
\newentry{sfS}{
  name=\ensuremath{\sym{sfS}_X(t)=1-\sym{cdfS}_X(t)},
  description={\Al{sf} of a \al{rv} $ X $.},
  text={survival function},
  type=symbols,
  sort={sf},
  symbol=\ensuremath{S}
}
\newentry{hrfS}{
  name=\ensuremath{\sym{hrfS}_X(t)=\dfrac{\sym{pdfS}_X(x)}{1-\sym{cdfS}_X(x)}},
  description={\Al{hrf} of a \al{rv} $X$.},
  text={hazard rate function},
  type=symbols,
  sort={hrf1},
  symbol=\ensuremath{h}
}
\newentry{mgfS}{
  name=\ensuremath{\sym{mgfS}_X(t)=\sym{E}(\e^{tX})},
  description={\Al{mgf} of a \al{rv} $ X $.},
  text={moment-generating function},
  type=symbols,
  sort={mgf},
  symbol=\ensuremath{M}
}
\newentry{cgfS}{
  name=\ensuremath{\sym{cgfS}_X(t)=\log\left[\sym{E}(\e^{tX})\right]},
  description={\Al{cgf} of a \al{rv} $ X $},
  text={cumulant-generating function},
  type=symbols,
  sort={cgf},
  symbol=\ensuremath{K}
}
\newentry{MKS}{
  name=\ensuremath{\sym{MKS}=\displaystyle\frac{\sum_{k=1}^{4}(-1)^k\sym{qfS}\left(\frac{2k-1}{8}\right)}{\sum_{k=1}^{2}(-1)^k\sym{qfS}\left(\frac{2k-1}{4}\right)}},
  description={\Al{MK} of implicit \al{rv}.},
  text={MK},
  type=symbols,
  sort={kurtosis2},
  symbol=\ensuremath{\mathcal{K}_{M}}
}
\newentry{BSS}{
  name=\ensuremath{\sym{BSS}=\displaystyle\frac{\sum_{k=1}^{3}(-1)^{k-1}\binom{2}{k}\sym{qfS}\left(\frac{2k-1}{4}\right)}{\sum_{k=1}^{2}(-1)^k\sym{qfS}\left(\frac{2k-1}{4}\right)}},
  description={\Al{BS} of implicit \al{rv}.},
  text={BS},
  type=symbols,
  sort={skewness2},
  symbol=\ensuremath{\mathcal{S}_{B}}
}
\newentry{llfS}{
  name=\ensuremath{\displaystyle\sym{llfS}(\sym{PV})= \sym{llfS}(\sym{PV}|\bm{x})=
  \sum_{i=1}^n\log[\sym{pdfS}_X(x_i|\sym{PV})]},
  description={\Al{llf} of $ \boldsymbol{\theta} $ given the data $ \bm{x} $},
  text={log-likelihood function},
  type=symbols,
  sort={lfllf},
  symbol=\ensuremath{\ell}
}
\newentry{lfS}{
  name=\ensuremath{\displaystyle\sym{lfS}(\sym{PV})=\sym{lfS}(\sym{PV}|\bm{x})=\prod_{i=1}^n\sym{pdfS}_X(x_i|\sym{PV})},
  description={\Al{lf} of $ \boldsymbol{\theta} $ given the data $ \bm{x} $},
  text={likelihood function},
  type=symbols,
  sort={lf},
  symbol=\ensuremath{\operatorname{L}}
}
\newentry{pllfS}{
  name=\ensuremath{\sym{llfS}_{\theta_1}(\sym{PV}) = \sym{llfS}(\sym{PV}|\bm{x},\theta_1=h(\theta_2,\ldots,\theta_p))},
  description={\Al{pllf} of $ \boldsymbol{\theta} $ given the data $ \bm{x} $ and $ \theta_1 $ expressed as a function $ h $ of the others parameters.},
  text={profile log-likelihood function},
  type=symbols,
  sort={lfprofile},
  symbol=\ensuremath{\sym{llf}_\alpha}
}
\newentry{pbefS}{
  name=\ensuremath{\sym{pbefS}(\sym{PV}) = \displaystyle\sum_{i=1}^{n}\left[\sym{qfS}(p_i)-x_{i:n}\right]^2},
  description={\Al{pbef} of $ \boldsymbol{\theta} $ given the data $ \bm{x} $},
  text={percentile-based estimation function},
  type=symbols,
  sort={pbef},
  symbol=\ensuremath{\mathfrak{p}}
}

%Definição de símbolos sem abreviaturas
\newentry{Pr}{
  name=\ensuremath{\sym{Pr}(E)},
  description={Probability of a \al{rv} $ E $},
  text={probability},
  type=symbols,
  category=symbol, %a categoria símbolo é usada quando não há abreviação
  sort={Pr},
  symbol=\ensuremath{\Pr}
}
\newentry{E}{
  name=\ensuremath{\displaystyle\sym{E}(X)=\int_{-\infty}^{\infty}x\sym{pdfS}_X(x)\,\mathrm{d}x},
  description={Expectation, or the expected value of a continuous \al{rv} $X$},
  text={expectation},
  type=symbols,
  category=symbol, %a categoria símbolo é usada quando não há abreviação
  sort={PrE},
  symbol=\ensuremath{\mathbb{E}}
}
\newentry{Var}{
  name=\ensuremath{\sym{Var}(X)=\sigma^2=\sym{E} [(X-\sym{mu})^2]},
  description={Variance of a \al{rv} $X$},
  text={variance},
  type=symbols,
  category=symbol, %a categoria símbolo é usada quando não há abreviação
  sort={PrEVar},
  symbol=\ensuremath{\operatorname{Var}}
}
\newentry{ncoms}{
  name=\ensuremath{\sym{ncoms} =\sym{E}(X^r)},
  description={$r$th ordinary moment of a \al{rv} $X$},
  text={$r$th non-central ordinary moment},
  type=symbols,
  category=symbol, %a categoria símbolo é usada quando não há abreviação
  sort={moment3},
  symbol=\ensuremath{\mu_r'}
}
\newentry{pwmS}{
  name=\ensuremath{\sym{pwmS} =\sym{E}\left(X^rF(X)^s[1-F(X)]^t\right)},
  description={$(r,s,t)$th \al{pwm} of \al{rv} $ X $.},
  text={$(r,s,t)$th \al{pwm}},
  type=symbols,
  category=symbol, %a categoria símbolo é usada quando não há abreviação
  sort={moment31},
  symbol=\ensuremath{\mu_{r,s,t}'}
}
\newentry{spwmS}{
  name=\ensuremath{\sym{spwmS} = \frac{1}{n}\sum_{i=1}^{n}\left(x_i^rF(x_i)^s[1-F(x_i)]^t\right)},
  description={$(r,s,t)$th sample \al{pwm} of \al{rv} $ X $.},
  text={$(r,s,t)$th sample \al{pwm}},
  type=symbols,
  category=symbol, %a categoria símbolo é usada quando não há abreviação
  sort={moment32},
  symbol=\ensuremath{\overline{X^r_{s,t}}}
}
\newentry{coms}{
  name=\ensuremath{\sym{coms} =\sym{E}([X-\sym{E}(X)]^r)},
  description={$r$th central ordinary moment of a \al{rv} $ X $.},
  text={c.o.m.},
  type=symbols,
  category=symbol, %a categoria símbolo é usada quando não há abreviação
  sort={moment2},
  symbol=\ensuremath{\mu_r}
}
\newentry{mu}{
  name=\ensuremath{\sym{mu}=\sym{E}(X)},
  description={Expected value of the \al{rv} $ X $.},
  text={moment},
  type=symbols,
  category=symbol, %a categoria símbolo é usada quando não há abreviação
  sort={moment1},
  symbol=\ensuremath{\mu}
}
\newentry{imS}{
  name=\ensuremath{\displaystyle\sym{imS}(x_0)=\int_{-\infty}^{x_0}x^r f_X(x)\,\mathrm{d}x},
  description={$r$th incomplete moment of a continuous \al{rv} $ X $.},
  text={i.m.},
  type=symbols,
  category=symbol, %a categoria símbolo é usada quando não há abreviação
  sort={moment4},
  symbol=\ensuremath{m_r}
}
\newentry{cum}{
  name=\ensuremath{\sym{cum}_1=\sym{cgfS}^{'}(0)},
  description={First cumulant},
  text={cumulants},
  category=symbol, %a categoria símbolo é usada quando não há abreviação
  type=symbols,
  sort={EUcum1},
  symbol=\ensuremath{\kappa}
}
\newentry{ncum}{
  name=\ensuremath{\sym{ncum}=\sym{cgfS}^{(n)}(0)},
  description={$n$th cumulant of a \al{rv} $X$},
  text={cumulants},
  category=symbol, %a categoria símbolo é usada quando não há abreviação
  type=symbols,
  sort={EUcum2},
  symbol=\ensuremath{\sym{cum}_n}	
}
\newentry{cumnlld}{
  name=\ensuremath{\sym{cumnlld}=\sym{E}\left(\sym{SC}_{\theta_1\cdots\theta_n}\right)},
  description={cumulant of the $n$th log-likelihood derivative.},
  text={cumulant of the $n$th log-likelihood derivative.},
  type=symbols,
  category=symbol, %a categoria símbolo é usada quando não há abreviação
  sort={EUcum3},
  symbol=\ensuremath{\sym{cum}_{\theta_1\cdots\theta_n}}
}
\newentry{cumj11}{
  name=\ensuremath{\sym{cumj11}=\sym{E}\left(\sym{SC}_{\theta_1}\cdots\sym{SC}_{\theta_n}\right)},
  description={Joint cumulant of the firsts log-likelihood derivatives.},
  text={joint cumulant of the firsts log-likelihood derivatives},
  type=symbols,
  category=symbol, %a categoria símbolo é usada quando não há abreviação
  sort={EUcum4},
  symbol=\ensuremath{\sym{cum}_{\theta_1,\ldots,\theta_n}}
}
\newentry{cumj12}{
  name=\ensuremath{\sym{cumj12}=\sym{E}\left(\sym{SC}_{\theta_1\theta_2}\sym{SC}_{\theta_3}\right)},
  description={Joint cumulant of the first and the second log-likelihood derivatives.},
  text={text},
  type=symbols,
  category=symbol, %a categoria símbolo é usada quando não há abreviação
  sort={EUcum5},
  symbol=\ensuremath{\sym{cum}_{\theta_1\theta_2,\theta_3}}
}
\newentry{cumj22}{
  name=\ensuremath{\sym{cumj22}=\sym{E}\left(\sym{SC}_{\theta_1\theta_2}\sym{SC}_{\theta_3\theta_4}\right)},
  description={Joint cumulant of the seconds log-likelihood derivatives.},
  text={text},
  type=symbols,
  category=symbol, %a categoria símbolo é usada quando não há abreviação
  sort={EUcum6},
  symbol=\ensuremath{\sym{cum}_{\theta_1\theta_2,\theta_3\theta_4}}
}
\newentry{cumj13}{
  name=\ensuremath{\sym{cumj13}=\sym{E}\left(\sym{SC}_{\theta_1}\sym{SC}_{\theta_2\theta_3\theta_4}\right)},
  description={Joint cumulant of the first and third log-likelihood derivatives.},
  text={text},
  type=symbols,
  category=symbol, %a categoria símbolo é usada quando não há abreviação
  sort={EUcum7},
  symbol=\ensuremath{\sym{cum}_{\theta_1,\theta_2\theta_3\theta_4}}
}
\newentry{cumj112}{
  name=\ensuremath{\sym{cumj112}=\sym{E}\left(\sym{SC}_{\theta_1}\sym{SC}_{\theta_2}\sym{SC}_{\theta_3\theta_4}\right)},
  description={Joint cumulant of the firsts and second log-likelihood derivatives.},
  text={joint cumulant},
  type=symbols,
  category=symbol, %a categoria símbolo é usada quando não há abreviação
  sort={EUcum8},
  symbol=\ensuremath{\sym{cum}_{\theta_1,\theta_2,\theta_3\theta_4}}
}
\newentry{invfei}{
  name=\ensuremath{\sym{invfei}^{\theta_1,\theta_j}},
  description={Inverse \al{fei} element.},
  text={inverse \al{fei}},
  type=symbols,
  category=symbol, %a categoria símbolo é usada quando não há abreviação
  sort={EUcum9},
  symbol=\ensuremath{\sym{cum}}
}
\newentry{dercum}{
  name=\ensuremath{\sym{dercum}=\frac{\partial}{\partial\theta_k}\,\sym{cum}_{\theta_i\theta_j}},
  description={First derivative of the cumulants with respect to the parameters.},
  text={first derivative of the cumulants with respect to the parameters},
  type=symbols,
  category=symbol, %a categoria símbolo é usada quando não há abreviação
  sort={EUcum10},
  symbol=\ensuremath{\sym{cum}_{\theta_i\theta_j}^{(\theta_k)}}
}
\newentry{skewness}{
  name=\ensuremath{\displaystyle\sym{skewness}=\frac{\sym{cum}_3}{\sym{cum}_2^{\nicefrac{3}{2}}}},
  description={Skewness},
  text={skewness},
  type=symbols,
  category=symbol, %a categoria símbolo é usada quando não há abreviação
  sort={skewness1},
  symbol=\ensuremath{\mathcal{S}}
}
\newentry{kurtosis}{
  name=\ensuremath{\sym{kurtosis}=\displaystyle\frac{\sym{cum}_4}{\sigma^4}},
  description={Kurtosis},
  text={kurtosis},
  type=symbols,
  category=symbol, %a categoria símbolo é usada quando não há abreviação
  sort={kurtosis1},
  symbol=\ensuremath{\mathcal{K}}
}
\newentry{median}{
  name=\ensuremath{\sym{median}=\sym{qfS}_X(\nicefrac{1}{2})},
  description={Median of a \al{rv} $ X $},
  text={median},
  type=symbols,
  category=symbol, %a categoria símbolo é usada quando não há abreviação
  sort={median},
  symbol=\ensuremath{\widetilde{M}}
}
\newentry{mode}{
  name=\ensuremath{\displaystyle\sym{mode}_X=\arg\max_{x} f_X(x)},
  description={Mode of \al{rv} $ X $},
  text={mode},
  type=symbols,
  category=symbol, %a categoria símbolo é usada quando não há abreviação
  sort={mode},
  symbol=\ensuremath{\operatorname{Mo}}
}
\newentry{igf}{
  name=\ensuremath{\displaystyle\sym{igf}(a,x)=\int_0^xt^{a-1}\e^{-t}\mathrm{d}t},
  description={Incomplete gamma\footnote{ab{aka} lower incomplete gamma} function},
  text={incomplete gamma function},
  type=symbols,
  category=symbol, %a categoria símbolo é usada quando não há abreviação
  sort={gf2},
  symbol=\ensuremath{\gamma}
}
\newentry{cigf}{
  name=\ensuremath{\displaystyle\sym{cigf}(a,x)=\int_x^{\infty} t^{a-1}\e^{-t}\mathrm{d}t},
  description={Complementary incomplete gamma\footnote{\ab{aka} upper incomplete gamma} function},
  text={complementary incomplete gamma function},
  type=symbols,
  category=symbol, %a categoria símbolo é usada quando não há abreviação
  sort={gf3},
  symbol=\ensuremath{\Gamma}
}
\newentry{pgf}{
  name=\ensuremath{\displaystyle\sym{pgf}^{(n)}(x)=\frac{\mathrm{d}^{n+1}}{\mathrm{d}x^{n+1}}\log\sym{gf}(x)},
  description={Polygamma function of order $n$.},
  text={polygamma function},
  type=symbols,
  category=symbol, %a categoria símbolo é usada quando não há abreviação
  sort={gf4},
  symbol=\ensuremath{\Psi}
}
\newentry{dgf}{
  name=\ensuremath{\displaystyle\sym{dgf}(x)=\frac{\mathrm{d}}{\mathrm{d}x}\log\sym{gf}(x)},
  description={Digamma function.},
  text={digamma function},
  type=symbols,
  category=symbol, %a categoria símbolo é usada quando não há abreviação
  sort={gf5},
  symbol=\ensuremath{\Psi}
}
\newentry{gf}{
  name=\ensuremath{\displaystyle\sym{gf}(a)=\int_0^{\infty} t^{a-1}\e^{-t}\mathrm{d}t},
  description={Gamma\footnote{\ab{aka} complete gamma} function},
  text={gamma function},
  type=symbols,
  category=symbol, %a categoria símbolo é usada quando não há abreviação
  sort={gf1},
  symbol=\ensuremath{\Gamma}
}
\newentry{bf}{
  name=\ensuremath{\displaystyle\sym{bf}(a,b)=\int_0^1t^{a-1}(1-t)^{b-1}\,\mathrm{d}t},
  description={Beta\footnote{\ab{aka} Euler integral of the first kind} function},
  text={beta function},
  type=symbols,
  category=symbol, %a categoria símbolo é usada quando não há abreviação
  sort={bf1},
  symbol=\ensuremath{\mathrm{B}}
}
\newentry{ibf}{
  name=\ensuremath{\displaystyle\sym{ibf}(x;a,b)=\int_0^xt^{a-1}(1-t)^{b-1}\,\mathrm{d}t},
  description={Incomplete beta\footnote{\ab{aka} lower incomplete beta} function},
  text={incomplete beta function},
  type=symbols,
  category=symbol, %a categoria símbolo é usada quando não há abreviação
  sort={bf2},
  symbol=\ensuremath{\mathrm{B}}
}
\newentry{mdmean}{
  name=\ensuremath{\sym{mdmean}=\sym{E}(|X-\sym{mu}|)},
  description={Mean deviations about the mean},
  text={mean deviation about the mean},
  type=symbols,
  category=symbol, %a categoria símbolo é usada quando não há abreviação
  sort={mean deviations about the mean},
  symbol=\ensuremath{\delta_{\sym{mu}}}
}
\newentry{mdmedian}{
  name=\ensuremath{\sym{mdmedian}=\sym{E}(|X-\sym{median}|)},
  description={Mean deviations about the median},
  text={mean deviation about the median},
  plural={mean deviations},
  type=symbols,
  category=symbol, %a categoria símbolo é usada quando não há abreviação
  sort={mean deviations about the median},
  symbol=\ensuremath{\delta_{\sym{median}}}
}
\newentry{Renyi}{
  name=\ensuremath{\displaystyle\sym{Renyi}(\rho)=\frac{1}{1-\rho}\log\left(\int_{-\infty}^{\infty}\sym{pdfS}(x)^\rho\,\mathrm{d}x\right)},
  description={Rényi entropy of a continuous \al{rv} $X$ with additional parameter $\rho>0$ and $\rho\ne 1$.},
  text={Rényi entropy},
  type=symbols,
  category=symbol, %a categoria símbolo é usada quando não há abreviação
  sort={entropy Rényi},
  symbol=\ensuremath{I_R}
}
\newentry{Tsallis}{
  name=\ensuremath{\displaystyle\sym{Tsallis}(q)=\frac{1}{q-1}\left(1-\int_{-\infty}^{\infty}\sym{pdfS}(x)^q\,\mathrm{d}x\right)},
  description={Tsallis entropy of a continuous \al{rv} $X$ with additional parameter $q\in\sym{Re}$ and $q\ne 1$.},
  text={Tsallis entropy},
  type=symbols,
  category=symbol, %a categoria símbolo é usada quando não há abreviação
  sort={entropy Tsallis},
  symbol=\ensuremath{I_T}
}
\newentry{Shannon}{
  name=\ensuremath{\displaystyle\sym{Shannon}=\sym{E}\left\{-\log[\sym{pdfS}(X)]\right\}},
  description={Shannon entropy\footnote{\ab{aka} Boltzmann-Gibbs entropy} of a continuous \al{rv} $X$.},
  text={Shannon entropy},
  plural={Shannon entropies},
  type=symbols,
  category=symbol, %a categoria símbolo é usada quando não há abreviação
  sort={entropy Shannon},
  symbol=\ensuremath{I_S}
}
\newentry{CrossShannon}{
  name=\ensuremath{\displaystyle\sym{CrossShannon}(X_1,X_2)=-\int_{-\infty}^{\infty} f_1(x)\log f_2(x)\,\mathrm{d}x},
  description={Cross Shannon entropy of a continuous \al{rv} $X_1$ relative to a \al{rv} $ X_2 $.},
  text={cross Shannon entropy},
  plural={cross Shannon entropies},
  type=symbols,
  category=symbol, %a categoria símbolo é usada quando não há abreviação
  sort={entropy Shannon cross},
  symbol=\ensuremath{I_{cS}}
}
\newentry{KLS}{
  name=\ensuremath{\displaystyle\sym{KLS}(X_1,X_2)=\int_{-\infty}^{\infty} f_1(x)\log\left[\frac{f_1(x)}{f_2(x)}\right](x)\,\mathrm{d}x},
  description={Kullback-Leibler divergence of a continuous \al{rv} $X_1$ relative to a \al{rv} $ X_2 $.},
  text={Kullback-Leibler divergence},
  type=symbols,
  category=symbol, %a categoria símbolo é usada quando não há abreviação
  sort={entropy Shannon KL},
  symbol=\ensuremath{\operatorname{KL}}
}
\newentry{KLdistS}{
  name=\ensuremath{\displaystyle\sym{KLdistS}(X_1,X_2)=\displaystyle\frac{\sym{KLS}(X_1,X_2)+\sym{KLS}(X_2,X_1)}{2}},
  description={Kullback-Leibler distance between $X_1$ and $ X_2 $.},
  text={Kullback-Leibler distance},
  type=symbols,
  category=symbol, %a categoria símbolo é usada quando não há abreviação
  sort={entropy Shannon distance},
  symbol=\ensuremath{d_{\sym{KLS}}}
}
\newentry{SV}{
  name=\ensuremath{\sym{SV}=\left(\sym{SC}_{\theta_1},\ldots,\sym{SC}_{\theta_n}\right)},
  description={Score vector relative to parameter vector $ \sym{PV}=(\theta_1,\ldots,\theta_n) $.},
  text={score vector},
  type=symbols,
  category=symbol, %a categoria símbolo é usada quando não há abreviação
  sort={score vector},
  symbol=\ensuremath{\bm{\sym{SC}}}
}
\newentry{SC}{
  name=\ensuremath{\displaystyle\sym{SC}_{\theta}=\frac{\partial\sym{llfS}(\sym{PV})}{\partial\theta}},
  description={Score vector component relative to parameter $\theta$.},
  text={score vector component},
  type=symbols,
  category=symbol, %a categoria símbolo é usada quando não há abreviação
  sort={score vector component},
  symbol=\ensuremath{U}
}
\newentry{SCD}{
  name=\ensuremath{\sym{SCD}=\displaystyle\frac{\partial\sym{llfS}(\sym{PV})}{\partial\theta_1\cdots\partial\theta_n}},
  description={Partial \al{llf} derivative relative to parameters $\theta_1,\ldots,\theta_n$.},
  text={score vector component derivative at an arbitrary points $\theta_1,\ldots,\theta_n$},
  type=symbols,
  category=symbol, %a categoria símbolo é usada quando não há abreviação
  sort={score vector component derivative},
  symbol=\ensuremath{\sym{SC}_{\theta_1\cdots\theta_n}}
}
\newentry{PS}{
  name=\ensuremath{\sym{PS}},
  description={Parameter space},
  text={parameter space},
  type=symbols,
  category=symbol, %a categoria símbolo é usada quando não há abreviação
  sort={parameter space},
  symbol=\ensuremath{\Theta}
}
\newentry{PV}{
  name=\ensuremath{\sym{PV}=\left(\theta_1,\ldots,\theta_n\right)},
  description={Parameter vector},
  text={parameter vector},
  type=symbols,
  category=symbol, %a categoria símbolo é usada quando não há abreviação
  sort={parameter vector},
  symbol=\ensuremath{\boldsymbol{\theta}}
}
\newentry{Delta}{
  name=\ensuremath{\sym{Delta}},
  description={Discriminant of a quadratic equation},
  long={discriminant}, %printed as \acrlong{}
  text={discriminant},
  type=symbols,
  category=symbol, %a categoria símbolo é usada quando não há abreviação
  sort={discriminant},
  symbol=\ensuremath{\Delta}
}
\newentry{foiS}{
  name=\ensuremath{\sym{foiS}_{i,j}=[\sym{foiS}(\sym{PV})]_{i,j}=\sym{SC}_{\theta_i\theta_j}},
  description={$i,j$th element of the \al{foi} matrix for $\boldsymbol{\theta}$},
  text={FOI},
  type=symbols,
  category=symbol, %a categoria símbolo é usada quando não há abreviação
  sort={foi1},
  symbol=\ensuremath{\operatorname{\bm{J}}}
}
\newentry{feiS}{
  name=\ensuremath{\sym{feiS}_{i,j}=[\sym{feiS}(\sym{PV})]_{i,j}=-\sym{cum}_{\theta_i\theta_j}},
  description={$i,j$th element of the \al{fei} matrix for $\boldsymbol{\theta}$},
  text={FEI},
  type=symbols,
  category=symbol, %a categoria símbolo é usada quando não há abreviação
  sort={fei1},
  symbol=\ensuremath{\operatorname{\bm{K}}}
}
\newentry{2F1}{
  name=\ensuremath{\sym{2F1}(a,b;c;x)=\displaystyle\sum_{k=0}^{\infty}\frac{(a)_k(b)_k}{(c)_k}\frac{x^k}{k!}},
  description={Gauss's hypergeometric function},
  long={Gauss's hypergeometric function}, %printed as \acrlong{}
  text={Gauss's hypergeometric function},
  type=symbols,
  category=symbol, %a categoria símbolo é usada quando não há abreviação
  sort={HF1},
  symbol=\ensuremath{_2\mathrm{F}_1}
}
\newentry{F1}{
  name=\ensuremath{\sym{F1}(a,b_1,b_2;c;x,y)=\displaystyle\sum_{i,j=0}^{\infty}\frac{(a)_{i+j}(b_1)_i(b_2)_j}{(c)_{i+j}}\frac{x^i}{i!}\frac{y^j}{j!}},
  description={first Appell's hypergeometric function},
  text={first Appell's hypergeometric function},
  type=symbols,
  category=symbol, %a categoria símbolo é usada quando não há abreviação
  sort={HF1Appell},
  symbol=\ensuremath{\mathrm{F}_1}
}
\newentry{Re}{
  name=\ensuremath{\sym{Re}},
  description={The set of real numbers},
  text={real numbers},
  type=symbols,
  sort={set Re},
  symbol=\ensuremath{\mathbb{R}}
}
\newentry{Z}{
  name=\ensuremath{\sym{Z}},
  description={The set of integers numbers},
  text={integers numbers},
  type=symbols,
  sort={set Z},
  symbol=\ensuremath{\mathbb{Z}}
}
\newentry{Im}{
  name=\ensuremath{\sym{Im}},
  description={The set of imaginary numbers},
  text={complex numbers},
  short={Im},
  type=symbols,
  sort={set Im},
  symbol=\ensuremath{\mathbb{I}}
}
\newentry{N}{
  name=\ensuremath{X\sim\sym{N}(\mu,\sigma^2)},
  description={$ X $ following normal distribution with mean $\mu$ and variance $\sigma^2$.},
  long={normal distribution},
  text={normal distribution},
  type=symbols,
  category=symbol, %a categoria símbolo é usada quando não há abreviação
  sort={normal},
  symbol=\ensuremath{\mathcal{N}}
}
\newentry{eqdef}{
  name=\sym{triangleq},
  description={Equal by definition},
  long={Equal by definition},
  text={Equal by definition},
  type=symbols,
  category=symbol, %a categoria símbolo é usada quando não há abreviação
  sort={equal},
  symbol=\ensuremath{\triangleq}
}
\newentry{Pochhammer}{
  name=\ensuremath{\sym{Pochhammer}=\displaystyle\frac{\Gamma(a+k)}{\Gamma(a)}},
  description={Pochhammer symbol.},
  text={Pochhammer symbol},
  type=symbols,
  category=symbol, %a categoria símbolo é usada quando não há abreviação
  sort={HF2},
  symbol=\ensuremath{(a)_k}
}
\newentry{EM}{
  name=\ensuremath{\displaystyle\sym{EM}=\lim_{n\to\infty}\left(-\log n + \sum_{k=1}^{n}\frac{1}{k}\right)},
  description={Euler-Mascheroni constant.},
  text={Euler-Mascheroni constant},
  type=symbols,
  category=symbol, %a categoria símbolo é usada quando não há abreviação
  sort={Euler–Mascheroni constant},
  symbol=\ensuremath{\bm{\gamma}}
}
\newentry{lpf}{
  name=\ensuremath{\displaystyle\sym{lpf}(x;s,a)=\sum_{n=0}^{\infty}\frac{x^n}{(n+a)^s}},
  description={Lerch transcendental Phi function.},
  text={Lerch transcendental Phi function},
  category=symbol,
  type=symbols,
  sort={lpf},
  symbol=\ensuremath{\bm{\Phi}}
}
\newentry{bias}{
  name=\ensuremath{\sym{bias}(\hat{\theta})=\sym{E}(\hat{\theta})},
  description={Bias of the estimative of $ \theta $.},
  text={bias},
  category=symbol,
  type=symbols,
  sort={bias},
  symbol=\ensuremath{\operatorname{Bias}}
}
\newentry{ospdfS}{
  name=\ensuremath{\sym{ospdfS}(x)=\displaystyle\frac{\sym{pdfS}(x)\sym{cdfS}(x)^{i-1}\sym{sfS}(x)^{n-i}}{\sym{bf}(i,n-i+1)}},
  description={\Al{pdf} of the $ i $th order statistic $ X_{i:n} $ for $ i=1,\ldots,n $},
  text={\as{pdf} of the $ i $th order statistic},
  category=symbols,
  type=symbols,
  sort={pdf20},
  symbol=\ensuremath{f_{i:n}}
}
\newentry{os}{
  name=\ensuremath{X_{1:n}\le\ldots\le X_{n:n}},
  description={$ i $th order statistic $ X_{i:n} $ for $ i=1,\ldots,n $},
  text={$ i $th order statistic},
  category=symbols,
  type=symbols,
  sort={pdf21},
  symbol=\ensuremath{X_{i:n}}
}

%Term definitions
\newabbr[longplural={characteristic functions},
shortplural={cfs}]{cf}{cf}{characteristic function}
\newabbr[longplural={probability density functions},
shortplural={pdfs}]{pdf}{pdf}{probability density function}
\newabbr[longplural={cumulative distribution functions},
shortplural={cdfs}]{cdf}{cdf}{cumulative distribution function}
\newabbr[longplural={quantile functions},
shortplural={qfs}]{qf}{qf}{quantile function}
\newabbr{sf}{sf}{survival function}
\newabbr[longplural={hazard rate functions},
shortplural={hrfs}]{hrf}{hrf}{hazard rate function}
\newabbr[longplural={reverse hazard rate functions},
shortplural={rhrfs}]{rhrf}{rhrf}{reverse hazard rate function}
\newabbr[longplural={moment-generating functions},
shortplural={mgfs}]{mgf}{mgf}{moment-generating function}
\newabbr[longplural={cumulant-generating functions},
shortplural={cgfs}]{cgf}{cgf}{cumulant-generating function}
\newabbr[longplural={maximum likelihood},
shortplural={ML}]{ML}{ML}{maximum likelihood}
\newabbr[longplural={maximum likelihood estimators},
shortplural={MLEs}]{MLE}{MLE}{maximum likelihood estimator}
\newabbr{CS-MLE}{CS-MLE}{Cox-Snell corrected \al{MLE}}
\newabbr[longplural={percentiles-based}]{PB}{PB}{percentile-based}
\newabbr{PBE}{PBE}{percentile-based estimator}
\newabbr{pbef}{pbef}{percentile-based estimation function}
\newabbr{ppbef}{ppbef}{profile percentile-based estimation function}
\newabbr[longplural={method of moments},shortplural={MM}]{MM}{MM}{method of moments}
\newabbr[longplural={least squares},shortplural={LS}]{LS}{LS}{least squares}
\newabbr[shortplural={WLS}]{WLS}{WLS}{weighted least squares}
\newabbr[longplural={profile log-likelihood functions},
shortplural={pllfs}]{pllf}{pllf}{profile log-likelihood function}
\newabbr[longplural={log-likelihood functions},
shortplural={llfs}]{llf}{llf}{log-likelihood function}
\newabbr[longplural={likelihood functions},
shortplural={lfs}]{lf}{lf}{likelihood function}
\newabbr{psf}{psf}{profile score function}
\newabbr[longplural={log-likelihood equations},
shortplural={lles}]{lle}{lle}{log-likelihood equation}
\newabbr[longplural={probability weighted moments},
shortplural={pwms}]{pwm}{pwm}{probability weighted moment}
\newabbr[longplural={order-statistics moments}]{osm}{osm}{order-statistics moment}
\newabbr[longplural={incomplete moments}]{im}{im}{incomplete moment}
\newabbr{Lm}{Lm}{$L$-moment}
\newabbr[prefix={the\space},
prefixfirst={the\space}]{BFGS}{BFGS}{Broyden–Fletcher–Goldfarb–Shanno algorithm}
\newabbr{MK}{MK}{Moors kurtosis}
\newabbr{BS}{BS}{Bowley Skewness}
\newabbr{KL}{KL}{Kullback-Leibler}
\newabbr{TTT}{TTT}{total time on test}
\newabbr{GoF}{GoF}{goodness-of-fit}
\newabbr{W*}{W*}{Cramér-von Mises}
\newabbr{A*}{A*}{Anderson Darling}
\newabbr{KS}{KS}{Kolmogorov-Smirnov}
\newabbr{AIC}{AIC}{Akaike Information Criterion}
\newabbr{BIC}{BIC}{Bayesian Information Criterion}
\newabbr{CAIC}{CAIC}{Consistent Akaike Information Criterion}
\newabbr{HQIC}{HQIC}{Hannan-Quinn Information Criterion}
\newabbr{ecdf}{ecdf}{empiriral cumulative density function}
\newabbr{SSD}{SSD}{sample standard deviation}
\newabbr{MSE}{MSE}{mean squared error}
\newabbr{foi}{OI}{observed information}
\newabbr{fei}{FIM}{Fisher information matrix}
\newabbr{rvi}{rvi}{regularly varying at infinity}



%\newabbr[longplural={moment generating functions}]{mgf}{mgf}{moment generating function}

%Families of distributions
\newabbr{EG-G}{EG-G}{exponentiated generalized}
\newabbr{Exp-G}{Exp-G}{exponentiated}
\newabbr{beta-G}{beta-G}{beta generalized}
\newabbr{gamma-G}{gamma-G}{gamma generalized}
\newabbr{Kw-G}{Kw-G}{Kumaraswamy generalized}
\newabbr{Weibull-G}{Weibull-G}{Weibull generalized}

%Distributions
\newabbr{EGNH}{EGNH}{exponentiated generalized Nadarajah-Haghighi}
\newabbr{ENH}{ENH}{exponentiated Nadarajah-Haghighi}
\newabbr{MNH}{MNH}{modified Nadarajah-Haghighi}
\newabbr{BNH}{BNH}{beta Nadarajah-Haghighi}
\newabbr{BBXII}{BBXII}{beta \al{BXII}}
\newabbr{MONH}{MONH}{Marshall-Olkin Nadarajah-Haghighi}
\newabbr{E2NH}{E2NH}{exponentiated (Leh\-mann type 2) Nadarajah-Haghighi}
\newabbr{ZBNH}{ZBNH}{Zografos-Balakrishnan Nadarajah-Haghighi}
\newabbr{TNH}{TNH}{transmuted Nadarajah-Haghighi}
\newabbr{PZBNH}{PZBNH}{Poisson Zografos-Balakrishnan Nadarajah-Haghighi}
\newabbr{NH}{NH}{Nadarajah-Haghighi's exponential}
\newabbr{EE}{EE}{exponentiated exponential}
\newabbr{EW}{EW}{exponentiated Weibull}
\newabbr{EG}{EG}{exponentiated gamma}
\newabbr{ELi}{EL}{exponentiated Lindley}
\newabbr{ELo}{ELo}{exponentiated Lomax}
%\newabbr{ER}{ER}{exponentiated Rayleigh}
\newabbr{ELL}{ELL}{exponentiated \al{LL}}
\newabbr{EBXII}{EBXII}{exponentiated \al{BXII}}
\newabbr{EHN}{EHN}{exponentiated half-normal}
\newabbr{GHN}{GHN}{generalized half-normal}
\newabbr{EHC}{EHC}{exponentiated half-Cauchy}
\newabbr{GHC}{GHC}{generalized half-Cauchy}
\newabbr{EGGa}{EGGa}{exponentiated generalized gamma}
\newabbr{BXII}{BXII}{Burr XII}
\newabbr{BX}{BX}{Burr X}
\newabbr{IN}{IN}{inverse normal}
\newabbr{IW}{IW}{inverse Weibull}
\newabbr{GG}{GG}{generalized gamma}
\newabbr{IG}{IG}{inverse gamma}
\newabbr{EGIN}{EGIN}{EG-inverse normal}
\newabbr{EGGG}{EGGG}{EG-generalized gaussian}
\newabbr{EGIW}{EGIW}{EG-inverse Weibull}
\newabbr{EGGu}{EGGu}{EG-Gumbel}
\newabbr{Gumbel}{Gu}{Gumbel}
\newabbr{gamma}{Ga}{gamma}
\newabbr{uniform}{U}{uniform}
\newabbr{Chen}{Ch}{Chen}
\newabbr{Weibull}{Wei}{Weibull}
\newabbr{q-Weibull}{q-We}{q-Weibull}
\newabbr{LN}{LN}{log-normal}
\newabbr{LL}{LL}{log-logistic}
\newabbr{LC}{LC}{log-Cauchy}
\newabbr{MP}{MP}{modified Perks}
\newabbr{KBessel}{K}{K-Bessel}
\newabbr[text=exponential]{Exp}{Exp}{exponential}
\newabbr[text=Rayleigh]{Rayleigh}{R}{Rayleigh}
\newabbr{GPW}{GPW}{generalized power Weibull}
\newabbr{KGPW}{KGPW}{Kumaraswamy \al{GPW}}
\newabbr{KNH}{KNH}{Kumaraswamy Nadarajah-Haghighi}
\newabbr{KBXII}{KBXII}{Kumaraswamy \al{BXII}}
\newabbr{KEBXII}{KEBXII}{Kumaraswamy exponentiated \al{BXII}}
\newabbr{KLL}{KLL}{Kumaraswamy \al{LL}}
\newabbr{ECR}{ECR}{exponentiated Cauchy-Rayleigh} 
\newabbr{SECR}{SECR}{squared exponentiated Cauchy-Rayleigh} 
\newabbr{ESCR}{ESCR}{exponentiated squared Cauchy-Rayleigh} 
\newabbr{CR}{CR}{Cauchy-Rayleigh}
\newabbr{SCR}{SCR}{squared Cauchy-Rayleigh}
%\newabbr{ECR}{ECR}{exponentiated Cauchy-Rayleigh}
\newabbr{Cauchy}{C}{Cauchy}
\newabbr{HTR}{HTR}{heavy-tailed Rayleigh}
\newabbr{McBXII}{McBXII}{McDonald \al{BXII}}
\newabbr{McLL}{McLL}{McDonald \al{LL}}
\newabbr{McLo}{McLo}{McDonald Lomax}
\newabbr{BLo}{BLo}{beta Lomax}
\newabbr{KLo}{KLo}{Kumaraswamy Lomax}
\newabbr{FP}{FP}{Feller-Pareto}
\newabbr{GFP}{GFP}{generalized Feller-Pareto}
\newabbr{GP}{GP}{generalized Pareto}
\newabbr{BSd}{BS}{Birnbaun-Saunders}
\newabbr{CW}{CW}{compound Weibull}
\newabbr{FW}{FW}{flexible Weibull}
\newabbr{TB}{TB}{transformed beta}
\newabbr{aS}{$\alpha$S}{$\alpha$-stable}
\newabbr{SaS}{S$\alpha$S}{symmetric $\alpha$-stable}
\newabbr{IaS}{I$\alpha$S}{isotropic $\alpha$-stable}
\newabbr{LE}{LE}{Lindley exponential}
\newabbr{SM}{SM}{Singh-Maddala}

%Others concepts
\newabbr{iid}{i.i.d.}{independent and identically distributed}
\newabbr{aka}{a.k.a.}{also known as}
\newabbr{ie}{i.e.}{\textit{id est}}
\newabbr{eg}{e.g.}{\textit{exampli gratia}}
\newabbr[shortplural={r.v.s}]{rv}{r.v.}{random variable}
\newabbr{iff}{iff}{if and only if}
\newabbr{itsm}{ITSM}{inverse transform sampling method}

%Acrônimos
\newabbr{SAR}{SAR}{synthetic aperture radar}
\newabbr{PolSAR}{PolSAR}{polarimetric synthetic aperture radar}

%Outros exemplos
\newabbr{html}{HTML}{hypertext markup language}
\newabbr{css}{CSS}{cascading style sheet}
\newabbr{xml}{XML}{extensible markup language}

